Nonparametric maximum likelihood methods for binary response models with random coefficients

Single index linear models for binary response with random coefficients have been extensively employed in many econometric settings under various parametric specifications of the distribution of the random coefficients. Nonparametric maximum likelihood estimation (NPMLE) as proposed by Cosslett (1983) and Ichimura and Thompson (1998), in contrast, has received less attention in applied work due primarily to computational difficulties. We propose a new approach to computation of NPMLEs for binary response models that significantly increase their computational tractability thereby facilitating greater flexibility in applications. Our approach, which relies on recent developments involving the geometry of hyperplane arrangements, is contrasted with the recently proposed deconvolution method of Gautier and Kitamura (2013). An application to modal choice for the journey to work in the Washington DC area illustrates the methods.

==> figures/GKTuning.tex <==
%latex.default(A, file = "GKTuning.tex", rgroup = paste(0:2, " Cars"),     n.rgroup = rep(7, 3), rowlabel = "T", caption = cap, caption.loc = "bottom",     label = "tab:GKTuning")%
\begin{table}[!tbp]
\begin{center}
\begin{tabular}{lrrrrr}
\hline\hline
\multicolumn{1}{l}{T}&\multicolumn{1}{c}{TX =  3}&\multicolumn{1}{c}{TX =  5}&\multicolumn{1}{c}{TX =  10}&\multicolumn{1}{c}{TX =  15}&\multicolumn{1}{c}{TX =  20}\tabularnewline
\hline
{\bfseries 0  Cars}&&&&&\tabularnewline
~~1&$ -39.33$&$ -41.27$&$ -40.94$&$ -41.54$&$ -41.13$\tabularnewline
~~2&$ -39.16$&$ -40.28$&$ -41.23$&$ -40.18$&$ -39.13$\tabularnewline
~~3&$ -39.54$&$ -40.64$&$ -40.75$&$ -39.51$&$ -39.07$\tabularnewline
~~4&$ -40.45$&$ -41.12$&$ -40.47$&$ -40.13$&$ -40.25$\tabularnewline
~~5&$ -41.29$&$ -41.83$&$ -41.02$&$ -41.19$&$ -41.58$\tabularnewline
~~7&$ -41.96$&$ -43.46$&$ -43.73$&$ -42.81$&$ -42.56$\tabularnewline
~~9&$ -42.81$&$ -45.48$&$ -47.13$&$ -45.96$&$ -45.25$\tabularnewline
\hline
{\bfseries 1  Cars}&&&&&\tabularnewline
~~1&$-223.33$&$-158.55$&$-178.90$&$-195.51$&$-163.35$\tabularnewline
~~2&$-179.44$&$-153.06$&$-157.35$&$-165.20$&$-153.68$\tabularnewline
~~3&$-145.51$&$-146.91$&$-162.93$&$-165.86$&$-166.01$\tabularnewline
~~4&$-148.49$&$-151.01$&$-162.31$&$-162.19$&$-180.44$\tabularnewline
~~5&$-151.37$&$-154.96$&$-169.23$&$-168.51$&$-198.44$\tabularnewline
~~7&$-161.38$&$-170.41$&$-191.81$&$-206.85$&$-229.93$\tabularnewline
~~9&$-168.29$&$-179.99$&$-198.82$&$-211.48$&$-230.02$\tabularnewline
\hline
{\bfseries 2  Cars}&&&&&\tabularnewline
~~1&$ -91.20$&$-164.31$&$-167.78$&$-126.56$&$ -93.70$\tabularnewline
~~2&$ -89.88$&$-126.42$&$-172.32$&$-143.76$&$-115.74$\tabularnewline
~~3&$-110.17$&$-141.13$&$-185.35$&$-165.72$&$-142.57$\tabularnewline
~~4&$-128.33$&$-152.74$&$-188.94$&$-162.99$&$-143.09$\tabularnewline
~~5&$-135.02$&$-154.10$&$-177.19$&$-148.85$&$-132.89$\tabularnewline
~~7&$-135.22$&$-146.45$&$-155.38$&$-132.70$&$-123.55$\tabularnewline
~~9&$-137.42$&$-145.49$&$-155.21$&$-139.99$&$-128.56$\tabularnewline
\hline
\end{tabular}
\caption{Log-likelihood of the Gautier-Kitamura estimator for various values of
the Fourier-Laplace series truncation parameters.}
\label{tab:GKTuning}
\end{center}
\end{table}


==> simulation/sim0a.tex <==
%latex.default(D, file = "sim0a.tex", rowlabel = "", where = "!htbp",     label = "tab.sim0a", caption = cap, caption.loc = "bottom")%
\begin{table}[!htbp]
\begin{center}
\begin{tabular}{lrrrr}
\hline\hline
\multicolumn{1}{l}{}&\multicolumn{1}{c}{GK}&\multicolumn{1}{c}{NPMLE}&\multicolumn{1}{c}{NPMLEs}&\multicolumn{1}{c}{Logit}\tabularnewline
\hline
MAE&$0.1211$&$0.0347$&$0.1064$&$0.1684$\tabularnewline
RMSE&$0.1532$&$0.0796$&$0.1428$&$0.2042$\tabularnewline
\hline
\end{tabular}
\caption{Bivariate Point Mass Simulation Setting:  
Mean Absolute and Root Mean Squared Errors of Predicted Probabilities\label{tab.sim0a}}\end{center}
\end{table}


==> simulation/sim1a.tex <==
%latex.default(D, file = "sim1a.tex", rowlabel = "", where = "!htbp",     label = "tab.sim1a", caption = cap, caption.loc = "bottom")%
\begin{table}[!htbp]
\begin{center}
\begin{tabular}{lrrrr}
\hline\hline
\multicolumn{1}{l}{}&\multicolumn{1}{c}{GK}&\multicolumn{1}{c}{NPMLE}&\multicolumn{1}{c}{NPMLEs}&\multicolumn{1}{c}{Logit}\tabularnewline
\hline
MAE&$0.1288$&$0.0592$&$0.0475$&$0.0709$\tabularnewline
RMSE&$0.1440$&$0.0748$&$0.0594$&$0.0896$\tabularnewline
\hline
\end{tabular}
\caption{Bivariate Gaussian Simulation Setting:  
Mean Absolute and Root Mean Squared Errors of Predicted Probabilities\label{tab.sim1a}}\end{center}
\end{table}

